UNCOVER: A NIRSpec Census of Lensed Galaxies at z=8.50-13.08 Probing a High AGN Fraction and Ionized Bubbles in the Shadow

We present JWST NIRSpec prism spectroscopy of gravitationally lensed galaxies at $z\gtrsim9$ found behind the massive galaxy cluster Abell 2744 in the UNCOVER Cycle 1 Treasury Program. We confirm the source redshift via emission lines and/or the Ly$\alpha$ break feature for ten galaxies at z=8.50-13.08 down to $M_{\rm UV}=-17.3$. We achieve a high confirmation rate of 100\% for $z>9$ candidates reported in Atek et al. (2023). Using six sources with multiple emission line detections, we find that the offset of the redshift estimates between the lines and the Ly$\alpha$ break alone with prism can be as large as $\pm0.2$, raising caution in designing future follow-up spectroscopy for the break-only sources with ALMA. With spec-$z$ confirmed sources in UNCOVER and the literature, we derive lower limits on the rest-frame ultraviolet (UV) luminosity function (LF) at $z\simeq9$-12 and find these lower limits to be consistent with recent photometric measurements. We identify at least two unambiguous and several possible active galactic nucleus (AGN) systems based on X-ray emission, broad line (BL) H$\beta$, high ionization line (e.g., NIV]1487, CIV1549) detections, and excess in UVLF. This requires the AGN LFs at $z\simeq$ 9-10 to be comparable or even higher than the X-ray AGN LF estimated at $z\sim6$ and indicates a plausible cause of the high abundance of $z>9$ galaxies claimed in recent photometric studies may be AGNs. One UV-luminous source is confirmed at the same redshift as a dusty BL AGN at $z=8.50$ with a physical separation of 380 kpc in the source plane. These two sources show blueward Ly$\alpha$ line or continuum emission, suggesting that they reside in the same ionized bubble with a radius of $7.69\pm0.18$ pMpc. Our results imply that AGNs have a non-negligible contribution to cosmic reionization.

==> latexdefs.tex <==
\def\farcm{% 
 \mbox{.\kern -0.7ex\raisebox{.9ex}{\scriptsize$\prime$}}% 
}% 
\def\farcs{% 
 \mbox{% 
  \kern  0.13ex.% 
  \kern -0.95ex\arcsec% 
  \kern -0.1ex% 
 }% 
}% 
%\renewcommand\case[2]{\mbox{$\frac{#1}{#2}$}}% 
%\renewcommand\slantfrac{\case}% 
\newcommand\onehalf{\slantfrac{1}{2}}% 
\newcommand\onethird{\slantfrac{1}{3}}% 
\newcommand\twothirds{\slantfrac{2}{3}}% 
\newcommand\onequarter{\slantfrac{1}{4}}% 
\newcommand\threequarters{\slantfrac{3}{4}}% 
\newcommand\ubvr{\mbox{$U\!BV\!R$}}%% UBVR system 
\newcommand\ub{\mbox{$U\!-\!B$}}%   % U-B 
\newcommand\bv{\mbox{$B\!-\!V$}}%   % B-V 
%\renewcommand\vr{\mbox{$V\!-\!R$}}%   % V-R 
\newcommand\ur{\mbox{$U\!-\!R$}}%   % U-R 
\makeatletter
\newcommand\ion[2]{#1$\;$\protect \textsmaller{\rmfamily\@Roman{#2}}}% 
\newcommand\smion[2]{#1$\;$\protect \footnotesize{\rmfamily\@Roman{#2}}\small}% 
\newcommand\scion[2]{#1$\;$\protect \tiny{\rmfamily\@Roman{#2}}\scriptsize}% 
\makeatother
\newcommand\nodata{ ~$\cdots$~ }% 
\newcommand\diameter{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}% 
\newcommand\degr{\arcdeg}% 
\newcommand\Sun{\sun}% 
\newcommand\Sol{\sun}% 
\newcommand\sun{\odot}% 
\newcommand\Mercury{\astro{\char1}}% Mercury symbol, "1" 
\newcommand\Venus{\astro{\char2}}% Venus symbol, "2" 
\newcommand\Earth{\earth}% 
\newcommand\Terra{\earth}% 
\newcommand\earth{\oplus}% 
\newcommand\Mars{\astro{\char4}}% Mars symbol, "4" 
\newcommand\Jupiter{\astro{\char5}}% Jupiter symbol, "5" 
\newcommand\Saturn{\astro{\char6}}% Saturn symbol, "6" 
\newcommand\Uranus{\astro{\char7}}% Uranus symbol, "7" 
\newcommand\Neptune{\astro{\char8}}% Neptune symbol, "8" 
\newcommand\Pluto{\astro{\char9}}% Pluo symbol, "9" 
\newcommand\Moon{\astro{\char10}}% Moon symbol, "M" 
\newcommand\Luna{\Moon}% 
\newcommand\Aries{\astro{\char11}}% 
\newcommand\VEq{\Aries}% vernal equinox (Aries) 
\newcommand\Taurus{\astro{\char12}}% 
\newcommand\Gemini{\astro{\char13}}% 
\newcommand\Cancer{\astro{\char14}}% 
\newcommand\Leo{\astro{\char15}}% 
\newcommand\Virgo{\astro{\char16}}% 
\newcommand\Libra{\astro{\char17}}% 
\newcommand\AEq{\Libra}% autumnal equinox (Libra) 
\newcommand\Scorpius{\astro{\char18}}% 
\newcommand\Sagittarius{\astro{\char19}}% 
\newcommand\Capricornus{\astro{\char20}}% 
\newcommand\Aquarius{\astro{\char21}}% 
\newcommand\Pisces{\astro{\char22}}% 

\newcommand\caii{Ca~{\sc ii}}
\newcommand\mgi{Mg~{\sc i}}
\newcommand\fehphot{$\rm{[Fe/H]_{phot}}$}
\newcommand\fehspec{$\rm{[Fe/H]_{spec}}$}
\newcommand\lcdm{$\Lambda$CDM}
\newcommand{\teff}{$T_{\rm{eff}}$}
\newcommand{\mathteff}{T_{\rm{eff}}}
\newcommand{\logg}{$\log g$}
\newcommand{\mathlogg}{\log g}
\newcommand{\feh}{[Fe/H]}
\newcommand{\mathfeh}{\rm{[Fe/H]}}
\newcommand{\afe}{[$\alpha$/Fe]}
\newcommand{\xfe}{[X/Fe]}
\newcommand{\mathafe}{\rm{[\alpha/Fe]}}
\newcommand{\mathxfe}{\rm{[X/Fe]}}
\newcommand{\ah}{[$\alpha$/H]}
\newcommand{\mathah}{\rm{[\alpha/H]}}
\newcommand{\vt}{$v_t$}
\newcommand{\mathvt}{v_t}
\newcommand{\cfht}{\textsc{cfht}}
\newcommand{\ha}{H$\alpha$}
\newcommand{\deep}{\textsc{deep2}}
\newcommand{\deimos}{\textsc{deimos}}
\newcommand{\mathaa}{\mathrm{\AA}}
\newcommand{\ngcaf}{NGC~1904 (M79)}
\newcommand{\ngca}{M79}
\newcommand{\ngcb}{NGC 2419}
\newcommand{\ngccf}{NGC~6205 (M13)}
\newcommand{\ngcc}{M13}
\newcommand{\ngcdf}{NGC~6838 (M71)}
\newcommand{\ngcd}{M71}
\newcommand{\ngce}{NGC 7006}
\newcommand{\ngcff}{NGC~7078 (M15)}
\newcommand{\ngcf}{M15}
\newcommand{\ngcg}{NGC 7492}
\newcommand{\bd}{BD+28$^{\circ}$~4211}

\newcommand{\otoprule}{\midrule[\heavyrulewidth]}

\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{Fund.~Cosmic~Phys.}
          % Fundamental Cosmic Physics
\newcommand\gca{Geochim.~Cosmochim.~Acta}
          % Geochimica Cosmochimica Acta
\newcommand\grl{Geophys.~Res.~Lett.}
          % Geophysics Research Letters
\newcommand\jcp{J.~Chem.~Phys.}
          % Journal of Chemical Physics
\newcommand\jgr{J.~Geophys.~Res.}
          % Journal of Geophysical Research
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{Nucl.~Phys.~A}
          % Nuclear Physics A
\newcommand\physrep{Phys.~Rep.}
          % Physics Reports
\newcommand\physscr{Phys.~Scr}
          % Physica Scripta
\newcommand\planss{Planet.~Space~Sci.}
          % Planetary Space Science
\newcommand\procspie{Proc.~SPIE}
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

